Dynamics of free group automorphisms

We present a coarse convexity result for the dynamics of free group automorphisms: Given an automorphism $\phi$ of a finitely generated free group $F$, we show that for all $x\in F$ and $0\leq i\leq N$, the length of $\phi^i(x)$ is bounded above by a constant multiple of the sum of the lengths of $x$ and $\phi^N(x)$, with the constant depending only on $\phi$.

==> bcc.tex <==
\section{Bounded cancellation}\label{bccsec}

Thurston's bounded cancellation lemma is one of the fundamental tools in this
paper. We state it in terms of homotopy equivalences of graphs.

\begin{lem}[Bounded cancellation lemma \cite{cooper}]\label{bcc}
Let $f:G\rightarrow G$ be a homotopy equivalence. There exists a constant
$\mathcal{C}_f$, depending only on $f$, with the property that for any
tight path $\rho$ in $G$ obtained by concatenating two paths $\alpha,
\beta$, we have
\[
\mathcal{L}(f_\#(\rho))\geq \mathcal{L}(f_\#(\alpha)) +
\mathcal{L}(f_\#(\beta)) - \mathcal{C}_f.
\]
\end{lem}

An upper bound for $\mathcal{C}_f$ can easily be read off from the map $f$
\cite{cooper}.  Let $f:G\rightarrow G$ be an improved relative train
track map with an exponentially growing stratum $H_r$ with growth rate
$\lambda_r$.  The {\em $r$-length} of a path $\rho$ in $G$,
$\mathcal{L}_r(\rho)$, is the total length of $\rho\cap H_r$.

If $\beta$ is an $r$-legal path in $G$ whose $r$-length satisfies
$\lambda_r \mathcal{L}_r(\beta)-2\mathcal{C}_f>\mathcal{L}_r(\beta)$ and
$\alpha, \gamma$ are paths such that the concatenation
$\alpha\beta\gamma$ is an immersion, then the $r$-length of the segment
in $f^k_\#(\alpha\beta\gamma)$ corresponding to $\beta$
(\convref{howtotighten}) will tend to infinity as $k$ tends to infinity.
The {\em critical length} $\mathcal{C}_r$ of $H_r$ is the infimum of the
lengths satisfying the above inequality, i.\ e.,
\begin{equation}
	\mathcal{C}_r=\frac{2\mathcal{C}_f}{\lambda_r-1}. \label{critlen}
\end{equation}



==> cor.tex <==
\section{Statements and corollaries}\label{corsec}

The following theorem is the main technical result of this paper.

\begin{thm}\label{mainthm}
Let $\phi\co F\rightarrow F$ be an an automorphism. Then there exists
an improved relative train track map representing some positive power of 
$\phi$ for which there exists a constant $K\geq 1$ with the following
property: For any pair of exponents $N,i$ satisfying $0\leq i \leq N$,
the following two statements hold:
\begin{enumerate}
\item If $\sigma$ is a circuit in $G$, then
\[
    \mathcal{L}\left(f^i_\#(\sigma)\right)\leq
    K\left(\mathcal{L}(\sigma)+\mathcal{L}\left(f^N_\#(\sigma)\right)\right).
\]
\item If $\rho$ is a path in $G$ that starts and ends at vertices, then
\[
    \mathcal{L}\left(f^i_\#(\rho)\right) \leq
    K\left(\mathcal{L}(\rho)+\mathcal{L}\left(f^N_\#(\rho)\right)\right).
\]
\end{enumerate}
Given the improved relative train track map $f\co G\rightarrow G,$ the
constant $K$ can be computed.
\end{thm}

We will present the proof of \thmref{mainthm} in \secref{polysec} and
\secref{pfsec}.  Right now, we show how \thmref{mainapp} follows from
\thmref{mainthm}.

\begin{proof}[Proof of \thmref{mainapp}]
Let $\phi\co F\rightarrow F$ be an automorphism of a finitely generated
free group $F=\langle x_1,\ldots,x_n\rangle$.
The first part of \thmref{mainthm} immediately implies that
the first part of \thmref{mainapp} holds for some positive power $\phi^k$,
i.e., there exists some $K'\geq 1$ such that for all $0\leq i\leq N$ and
$w\in F$, we have
\[
    ||\phi^{ik}_\#(w)||\leq K'\left(||w||+||\phi^{Nk}_\#(w)||\right),
\]
where we compute lengths with respect to the generators $x_1,\ldots,x_n$.

Let $L=\max\{|\phi(x_i)|\}$. Then, for $0\leq j<k$, we have
\[
	L^{-k}||\phi^{ik+j}(w)||\leq ||\phi^{ik}(w)||\leq L^k||\phi^{ik+j}(w)||
\]
for all $w\in F$. We conclude that for all $0\leq i\leq N$ and $w\in F$,
we have
\[
    L^{-k}||\phi^{i}_\#(w)||\leq K'\left(||w||+L^k||\phi^N_\#(w)||\right),
\]
so that the first part of \thmref{mainapp} holds with $K=L^{2k}K'$.

In order to prove the second assertion, we modify a trick from \cite{bfgafa2}.
Let $F'$ be the free group generated by $x_1,\ldots,x_n$ and an additional
generator $a$. We define an automorphism $\psi\co F'\rightarrow F'$ by
letting $\psi(x_i)=\phi(x_i)$ for all $1\leq i\leq n$, and $\psi(a)=a$.

By the previous step, the first part of \thmref{mainapp} holds for $\psi$,
with some constant $K'\geq 1$. Let $w$ be some word in $F$. Then, for all
$i\geq 0$, $\psi^i(aw)$ is a cyclically reduced word in $F'$, so that we
have $|\phi^i(w)|+1=||\psi^i(aw)||$. We conclude that
\[
	|\phi^i(w)|+1\leq K'(|w|+|\phi^N(w)|+2),
\]
for all $0\leq i\leq N$. Now the second assertion of \thmref{mainapp}
holds with $K=2K'$.
\end{proof}


